Inelastic dark matter scattering off Thallium cannot save DAMA

We study the compatibility of the observed DAMA modulation signal with inelastic scattering of dark matter (DM) off of the $0.1\%$ Thallium (Tl) dopant in DAMA. In this work we test whether there exist regions of parameter space where the Tl interpretation gives a good fit to the most recent data from DAMA, and whether these regions are compatible with the latest constraints from other direct detection experiments. Previously, Chang et al. in 2010, had proposed the Tl interpretation of the DAMA data, and more recently (in 2019) the DAMA/LIBRA collaboration found regions in parameter space of Tl inelastic scattering that differ by more than $10\sigma$ from a no modulation hypothesis. We have expanded upon their work by testing whether the regions of parameter space where inelastic DM-Tl scattering gives a good fit to the most recent DAMA data survive the constraints placed by the lack of a DM signal in XENON1T and CRESST-II. In addition, we have tested how these regions change with the main sources of uncertainty: the Tl quenching factor, which has never been measured directly, and the astrophysical uncertainties in the DM distribution. We conclude that inelastic DM scattering off Tl cannot explain the DAMA data in light of null results from other experiments.

==> previousbib.tex <==
\begin{comment}
\begin{thebibliography}{99}

%\cite{Goodman:1984dc}
\bibitem{Goodman:1984dc} 
  M.~W.~Goodman and E.~Witten,
  %``Detectability of Certain Dark Matter Candidates,''
  Phys.\ Rev.\ D {\bf 31}, 3059 (1985).
  doi:10.1103/PhysRevD.31.3059
  %%CITATION = doi:10.1103/PhysRevD.31.3059;%%
  %1055 citations counted in INSPIRE as of 24 Aug 2018

%\cite{Drukier:1986tm}
\bibitem{Drukier:1986tm} 
  A.~K.~Drukier, K.~Freese and D.~N.~Spergel,
  %``Detecting Cold Dark Matter Candidates,''
  Phys.\ Rev.\ D {\bf 33}, 3495 (1986).
  doi:10.1103/PhysRevD.33.3495
  %%CITATION = doi:10.1103/PhysRevD.33.3495;%%
  %712 citations counted in INSPIRE as of 24 Sep 2018

%\cite{Bozorgnia:2016fjt}
\bibitem{Bozorgnia:2016fjt} 
  N.~Bozorgnia {\it et al.},
  %``Predictions of hydrodynamic simulations for direct dark matter detection,''
  J.\ Phys.\ Conf.\ Ser.\  {\bf 718}, no. 4, 042007 (2016).
  doi:10.1088/1742-6596/718/4/042007
  %%CITATION = doi:10.1088/1742-6596/718/4/042007;%%
  %1 citations counted in INSPIRE as of 04 Oct 2018
  
  %\cite{Kelso:2016qqj}
\bibitem{Kelso:2016qqj} 
  C.~Kelso, C.~Savage, M.~Valluri, K.~Freese, G.~S.~Stinson and J.~Bailin,
  %``The impact of baryons on the direct detection of dark matter,''
  JCAP {\bf 1608}, 071 (2016)
  doi:10.1088/1475-7516/2016/08/071
  [arXiv:1601.04725 [astro-ph.GA]].
  %%CITATION = doi:10.1088/1475-7516/2016/08/071;%%
  %39 citations counted in INSPIRE as of 04 Oct 2018
  
  %\cite{Sloane:2016kyi}
\bibitem{Sloane:2016kyi} 
  J.~D.~Sloane, M.~R.~Buckley, A.~M.~Brooks and F.~Governato,
  %``Assessing Astrophysical Uncertainties in Direct Detection with Galaxy Simulations,''
  Astrophys.\ J.\  {\bf 831}, 93 (2016)
  doi:10.3847/0004-637X/831/1/93
  [arXiv:1601.05402 [astro-ph.GA]].
  %%CITATION = doi:10.3847/0004-637X/831/1/93;%%
  %36 citations counted in INSPIRE as of 04 Oct 2018

  %\cite{Green:2002ht}
\bibitem{Green:2002ht} 
  A.~M.~Green,
  %``Effect of halo modeling on WIMP exclusion limits,''
  Phys.\ Rev.\ D {\bf 66}, 083003 (2002)
  doi:10.1103/PhysRevD.66.083003
  [astro-ph/0207366].
  %%CITATION = doi:10.1103/PhysRevD.66.083003;%%
  %89 citations counted in INSPIRE as of 29 Mar 2019
  
  %\cite{McCabe:2010zh}
\bibitem{McCabe:2010zh} 
  C.~McCabe,
  %``The Astrophysical Uncertainties Of Dark Matter Direct Detection Experiments,''
  Phys.\ Rev.\ D {\bf 82}, 023530 (2010)
  doi:10.1103/PhysRevD.82.023530
  [arXiv:1005.0579 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.82.023530;%%
  %159 citations counted in INSPIRE as of 29 Mar 2019
  
%\cite{Fairbairn:2012zs}
\bibitem{Fairbairn:2012zs} 
  M.~Fairbairn, T.~Douce and J.~Swift,
  %``Quantifying Astrophysical Uncertainties on Dark Matter Direct Detection Results,''
  Astropart.\ Phys.\  {\bf 47}, 45 (2013)
  doi:10.1016/j.astropartphys.2013.06.003
  [arXiv:1206.2693 [astro-ph.CO]].
  %%CITATION = doi:10.1016/j.astropartphys.2013.06.003;%%
  %45 citations counted in INSPIRE as of 29 Mar 2019  
  
%\cite{Benito:2016kyp}
\bibitem{Benito:2016kyp} 
  M.~Benito, N.~Bernal, N.~Bozorgnia, F.~Calore and F.~Iocco,
  %``Particle Dark Matter Constraints: the Effect of Galactic Uncertainties,''
  JCAP {\bf 1702}, no. 02, 007 (2017)
  Erratum: [JCAP {\bf 1806}, no. 06, E01 (2018)]
  doi:10.1088/1475-7516/2017/02/007, 10.1088/1475-7516/2018/06/E01
  [arXiv:1612.02010 [hep-ph]].
  %%CITATION = doi:10.1088/1475-7516/2017/02/007, 10.1088/1475-7516/2018/06/E01;%%
  %25 citations counted in INSPIRE as of 29 Mar 2019  

%\cite{Green:2017odb}
\bibitem{Green:2017odb} 
  A.~M.~Green,
  %``Astrophysical uncertainties on the local dark matter distribution and direct detection experiments,''
  J.\ Phys.\ G {\bf 44}, no. 8, 084001 (2017)
  doi:10.1088/1361-6471/aa7819
  [arXiv:1703.10102 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1361-6471/aa7819;%%
  %18 citations counted in INSPIRE as of 30 Aug 2018  
  
%\cite{Fowlie:2017ufs}
\bibitem{Fowlie:2017ufs} 
  A.~Fowlie,
  %``Halo-independence with quantified maximum entropy at DAMA/LIBRA,''
  JCAP {\bf 1710}, no. 10, 002 (2017)
  doi:10.1088/1475-7516/2017/10/002
  [arXiv:1708.00181 [hep-ph]].
  %%CITATION = doi:10.1088/1475-7516/2017/10/002;%%
  %5 citations counted in INSPIRE as of 25 Apr 2019  
  
%\cite{Ibarra:2018yxq}
\bibitem{Ibarra:2018yxq} 
  A.~Ibarra, B.~J.~Kavanagh and A.~Rappelt,
  %``Bracketing the impact of astrophysical uncertainties on local dark matter searches,''
  JCAP {\bf 1812}, no. 12, 018 (2018)
  doi:10.1088/1475-7516/2018/12/018
  [arXiv:1806.08714 [hep-ph]].
  %%CITATION = doi:10.1088/1475-7516/2018/12/018;%%
  %6 citations counted in INSPIRE as of 29 Mar 2019  
 
 %\cite{Fowlie:2018svr}
\bibitem{Fowlie:2018svr} 
  A.~Fowlie,
  %``Non-parametric uncertainties in the dark matter velocity distribution,''
  JCAP {\bf 1901}, no. 01, 006 (2019)
  doi:10.1088/1475-7516/2019/01/006
  [arXiv:1809.02323 [hep-ph]].
  %%CITATION = doi:10.1088/1475-7516/2019/01/006;%%
  %2 citations counted in INSPIRE as of 25 Apr 2019

%\cite{Petac:2018wnu}
\bibitem{Petac:2018wnu} 
  M.~Petač and P.~Ullio,
  %``Two-integral distribution functions in axisymmetric galaxies: implications for dark matter searches,''
  Phys.\ Rev.\ D {\bf 99}, no. 4, 043003 (2019)
  doi:10.1103/PhysRevD.99.043003
  [arXiv:1812.01531 [astro-ph.GA]].
  %%CITATION = doi:10.1103/PhysRevD.99.043003;%%

%\cite{Necib:2018iwb}
\bibitem{Necib:2018iwb} 
  L.~Necib, M.~Lisanti and V.~Belokurov,
  %``Dark Matter in Disequilibrium: The Local Velocity Distribution from SDSS-Gaia,''
  arXiv:1807.02519 [astro-ph.GA].
  %%CITATION = ARXIV:1807.02519;%%
  %3 citations counted in INSPIRE as of 04 Oct 2018

%\cite{Evans:2018bqy}
\bibitem{Evans:2018bqy} 
  N.~W.~Evans, C.~A.~J.~O'Hare and C.~McCabe,
  %``Refinement of the standard halo model for dark matter searches in light of the Gaia Sausage,''
  Phys.\ Rev.\ D {\bf 99}, no. 2, 023012 (2019)
  doi:10.1103/PhysRevD.99.023012
  [arXiv:1810.11468 [astro-ph.GA]].
  %%CITATION = doi:10.1103/PhysRevD.99.023012;%%
  %10 citations counted in INSPIRE as of 16 May 2019

%\cite{Salucci:2010qr}
\bibitem{Salucci:2010qr} 
  P.~Salucci, F.~Nesti, G.~Gentile and C.~F.~Martins,
  %``The dark matter density at the Sun's location,''
  Astron.\ Astrophys.\  {\bf 523}, A83 (2010)
  doi:10.1051/0004-6361/201014385
  [arXiv:1003.3101 [astro-ph.GA]].
  %%CITATION = doi:10.1051/0004-6361/201014385;%%
  %255 citations counted in INSPIRE as of 04 Oct 2018
  
 %\cite{Catena:2009mf}
\bibitem{Catena:2009mf} 
  R.~Catena and P.~Ullio,
  %``A novel determination of the local dark matter density,''
  JCAP {\bf 1008}, 004 (2010)
  doi:10.1088/1475-7516/2010/08/004
  [arXiv:0907.0018 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2010/08/004;%%
  %409 citations counted in INSPIRE as of 04 Oct 2018

 %\cite{Weber:2010}
\bibitem{Weber:2010}
  M.~Weber and W.~de~Boer,
  %``Determination of the local dark matter density in our Galaxy,''
  A \& A {\bf 509}, A25 (2010)
  doi:10.1051/0004-6361/200913381
  [arXiv:0910.4272 [astro-ph.CO]].

%\cite{Iocco:2011jz}
\bibitem{Iocco:2011jz} 
  F.~Iocco, M.~Pato, G.~Bertone and P.~Jetzer,
  %``Dark Matter distribution in the Milky Way: microlensing and dynamical constraints,''
  JCAP {\bf 1111}, 029 (2011)
  doi:10.1088/1475-7516/2011/11/029
  [arXiv:1107.5810 [astro-ph.GA]].
  %%CITATION = doi:10.1088/1475-7516/2011/11/029;%%
  %141 citations counted in INSPIRE as of 04 Oct 2018
  
 %\cite{McMillan:2011}
\bibitem{McMillan:2011}
  P.~J.~McMillan,
  %``Mass models of the Milky Way,''
  MNRAS {\bf 414}, 2446 (2011)
  doi:10.1111/j.1365-2966.2011.18564.x
  [arXiv:1102.4340 [astro-ph.GA]].  
  
%\cite{Pato:2015dua}
\bibitem{Pato:2015dua} 
  M.~Pato, F.~Iocco and G.~Bertone,
  %``Dynamical constraints on the dark matter distribution in the Milky Way,''
  JCAP {\bf 1512}, no. 12, 001 (2015)
  doi:10.1088/1475-7516/2015/12/001
  [arXiv:1504.06324 [astro-ph.GA]].
  %%CITATION = doi:10.1088/1475-7516/2015/12/001;%%
  %65 citations counted in INSPIRE as of 04 Oct 2018  

%\cite{McKee:2015hwa}
\bibitem{McKee:2015hwa} 
  C.~F.~McKee, A.~Parravano and D.~J.~Hollenbach,
  %``Stars, Gas, and Dark Matter in the Solar Neighborhood,''
  Astrophys.\ J.\  {\bf 814}, no. 1, 13 (2015)
  doi:10.1088/0004-637X, 10.1088/0004-637X/814/1/13
  [arXiv:1509.05334 [astro-ph.GA]].
  %%CITATION = doi:10.1088/0004-637X, 10.1088/0004-637X/814/1/13;%%
  %45 citations counted in INSPIRE as of 03 Apr 2019 
  
%\cite{Xia:2015agz}
\bibitem{Xia:2015agz} 
  Q.~Xia {\it et al.},
  %``Determining the local dark matter density with LAMOST data,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 458}, no. 4, 3839 (2016)
  doi:10.1093/mnras/stw565
  [arXiv:1510.06810 [astro-ph.GA]].
  %%CITATION = doi:10.1093/mnras/stw565;%%
  %15 citations counted in INSPIRE as of 03 Apr 2019  

 %\cite{Huang:2016}
\bibitem{Huang:2016}
  Y.~Huang,  X.~W.~Liu, H.~B.~Yuan, M.~S.~Xiang, H.~W.~Zhang,  B.~Q.~Chen, J.~J.~Ren, C.~Wang,  Y.~Zhang, Y.~H.~Hou, Y.~F.~Wang and  Z.~H.~Cao,
  %``The Milky Way's rotation curve out to 100 kpc and its constraint on the Galactic mass distribution,''
  MNRAS {\bf 463}, 2623 (2016)
  doi:10.1093/mnras/stw2096
  [arXiv:1604.01216 [astro-ph.GA]].    
  
 %\cite{McMillan:2016}
\bibitem{McMillan:2016}
  P.~J.~McMillan,
  %``The mass distribution and gravitational potential of the Milky Way,''
  MNRAS {\bf 465}, 76 (2017)
  doi:10.1093/mnras/stw2759
  [arXiv:1608.00971 [astro-ph.GA]].    
     
  
%\cite{Sivertsson:2017rkp}
\bibitem{Sivertsson:2017rkp} 
  S.~Sivertsson, H.~Silverwood, J.~I.~Read, G.~Bertone and P.~Steger,
  %``The localdark matter density from SDSS-SEGUE G-dwarfs,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 478}, no. 2, 1677 (2018)
  doi:10.1093/mnras/sty977
  [arXiv:1708.07836 [astro-ph.GA]].
  %%CITATION = doi:10.1093/mnras/sty977;%%
  %21 citations counted in INSPIRE as of 03 Apr 2019  
 
  
%\cite{Buch:2018qdr}
\bibitem{Buch:2018qdr} 
  J.~Buch, J.~S.~C.~Leung and J.~Fan,
  %``Using Gaia DR2 to Constrain Local Dark Matter Density and Thin Dark Disk,''
  arXiv:1808.05603 [astro-ph.GA].
  %%CITATION = ARXIV:1808.05603;%%
  %8 citations counted in INSPIRE as of 03 Apr 2019  
  
%\cite{Widmark:2018ylf}
\bibitem{Widmark:2018ylf} 
  A.~Widmark,
  %``Measuring the local matter density using Gaia DR2,''
  Astron.\ Astrophys.\  {\bf 623}, A30 (2019)
  doi:10.1051/0004-6361/201834718
  [arXiv:1811.07911 [astro-ph.GA]].
  %%CITATION = doi:10.1051/0004-6361/201834718;%%
  %1 citations counted in INSPIRE as of 03 Apr 2019  
  
  %\cite{deSalas:2019}
\bibitem{deSalas:2019} 
  P.~F.~de Salas, K.~Malhan, K.~Freese, K.~Hattori and M.~Valluri,
  %``On the estimation of the Local Dark Matter Density using the rotation curve of the Milky Way,''
  in preparation.
  
  
%\cite{Workgroup:2017lvb}
\bibitem{Workgroup:2017lvb} 
  T.~Bringmann {\it et al.} [The GAMBIT Dark Matter Workgroup],
  %``DarkBit: A GAMBIT module for computing dark matter observables and likelihoods,''
  Eur.\ Phys.\ J.\ C {\bf 77}, no. 12, 831 (2017)
  doi:10.1140/epjc/s10052-017-5155-4
  [arXiv:1705.07920 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-5155-4;%%
  %43 citations counted in INSPIRE as of 10 Sep 2018  
  
%\cite{Aprile:2017iyp}
\bibitem{Aprile:2017iyp} 
  E.~Aprile {\it et al.} [XENON Collaboration],
  %``First Dark Matter Search Results from the XENON1T Experiment,''
  Phys.\ Rev.\ Lett.\  {\bf 119}, no. 18, 181301 (2017)
  doi:10.1103/PhysRevLett.119.181301
  [arXiv:1705.06655 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevLett.119.181301;%%
  %480 citations counted in INSPIRE as of 04 Oct 2018

%\cite{Piffl:2013mla}
\bibitem{Piffl:2013mla} 
  T.~Piffl {\it et al.},
  %``The RAVE survey: the Galactic escape speed and the mass of the Milky Way,''
  Astron.\ Astrophys.\  {\bf 562}, A91 (2014)
  doi:10.1051/0004-6361/201322531
  [arXiv:1309.4293 [astro-ph.GA]].
  %%CITATION = doi:10.1051/0004-6361/201322531;%%
  %114 citations counted in INSPIRE as of 30 Aug 2018

\bibitem{Monari:2018}
  G.~Monari {\it et al.},
  %``The escape speed curve of the Galaxy obtained from Gaia DR2 implies a heavy Milky Way,''
  Astron.\ Astrophys.\  {\bf 616}, L9 (2018)
  doi:10.1051/0004-6361/201833748
  [arXiv:1807.04565 [astro-ph.GA]].
  %%CITATION = doi:10.1051/0004-6361/201833748;%%

%\cite{Lavalle:2014rsa}
\bibitem{Lavalle:2014rsa} 
  J.~Lavalle and S.~Magni,
  %``Making sense of the local Galactic escape speed estimates in direct dark matter searches,''
  Phys.\ Rev.\ D {\bf 91}, no. 2, 023510 (2015)
  doi:10.1103/PhysRevD.91.023510
  [arXiv:1411.1325 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevD.91.023510;%%
  %17 citations counted in INSPIRE as of 29 Mar 2019

%\cite{Read:2014qva}
\bibitem{Read:2014qva} 
  J.~I.~Read,
  %``The Local Dark Matter Density,''
  J.\ Phys.\ G {\bf 41}, 063101 (2014)
  doi:10.1088/0954-3899/41/6/063101
  [arXiv:1404.1938 [astro-ph.GA]].
  %%CITATION = doi:10.1088/0954-3899/41/6/063101;%%
  %218 citations counted in INSPIRE as of 29 Aug 2019

  %\cite{Mroz2019}
\bibitem{Mroz2019}
 P.~Mr{\'{o}}z, A.~Udalski, D.~M.~Skowron, J.~Skowron, I.~Soszy{\'{n}}ski, P.~Pietrukowicz, M.~K.~Szyma{\'{n}}ski, R.~Poleski , S.~Koz{\l}owski and K.~Ulaczyk
  %``Rotation Curve of the Milky Way from Classical Cepheids,''
  Astrophys.\ J.\  {\bf 870}, L10 (2019)
  doi:10.3847/2041-8213/aaf73f
  [arXiv:1810.02131 [astro-ph.GA]].

  %\cite{Eilers2019}
\bibitem{Eilers2019}
 A.~Eilers, D.~W.~Hogg, H.~Rix and M.~K.~Ness,
  %``The Circular Velocity Curve of the Milky Way from 5 to 25 kpc,''
  Astrophys.\ J.\  {\bf 871}, 120 (2019)
  doi:10.3847/1538-4357/aaf648
  [arXiv:1810.09466 [astro-ph.GA]].

%\cite{Reid:2004rd}
\bibitem{Reid:2004rd} 
  M.~J.~Reid and A.~Brunthaler,
  %``The Proper motion of Sgr A*. 2. The Mass of Sgr A*,''
  Astrophys.\ J.\  {\bf 616}, 872 (2004)
  doi:10.1086/424960
  [astro-ph/0408107].
  %%CITATION = doi:10.1086/424960;%%
  %284 citations counted in INSPIRE as of 30 Apr 2019
  
%\cite{Abuter:2018drb}
\bibitem{Abuter:2018drb} 
  R.~Abuter {\it et al.} [GRAVITY Collaboration],
  %``Detection of the gravitational redshift in the orbit of the star S2 near the Galactic centre massive black hole,''
  Astron.\ Astrophys.\  {\bf 615}, L15 (2018)
  doi:10.1051/0004-6361/201833718
  [arXiv:1807.09409 [astro-ph.GA]].
  %%CITATION = doi:10.1051/0004-6361/201833718;%%
  %41 citations counted in INSPIRE as of 30 Apr 2019  

%\cite{Abuter:2019}
\bibitem{Abuter:2019} 
  R.~Abuter {\it et al.} [GRAVITY Collaboration],
  %``A geometric distance measurement to the Galactic Center black hole with 0.3\% uncertainty,''
  [arXiv:1904.05721 [astro-ph.GA]].

  
%\cite{Barlow:2004wg}
\bibitem{Barlow:2004wg} 
  R.~Barlow,
  %``Asymmetric statistical errors,''
  physics/0406120.
  %%CITATION = PHYSICS/0406120;%%
  %34 citations counted in INSPIRE as of 30 Aug 2018

 %\cite{Deason:2019}
\bibitem{Deason:2019}
  A.~J.~Deason, A.~Fattahi, V.~Belokurov, N.~W.~Evans, R.~J.~J.~Grand, F.~Marinacci and R.~Pakmor,
  %``The local high velocity tail and the Galactic escape speed,''
  MNRAS {\bf 485}, 3514 (2019)
  doi:10.1093/mnras/stz623
  [arXiv:1901.02016 [astro-ph.GA]]. 

  
\bibitem{Chang:2010pr} 
  S.~Chang, R.~F.~Lang and N.~Weiner,
  %``Effect of Thallium Impurities in the DAMA Experiment on the Allowed Parameter Space for Inelastic Dark Matter,''
  Phys.\ Rev.\ Lett.\  {\bf 106}, 011301 (2011)
  doi:10.1103/PhysRevLett.106.011301
  [arXiv:1007.2688 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.106.011301;%%
  %54 citations counted in INSPIRE as of 24 Mar 2020
  
\bibitem{Koposov_2010}
    S.~E.~Koposov, H.~Rix, and D.~W.~Hogg, 
    The Astrophys. J. {\bf712.1} (2010)\\
    doi: 10.1088/0004-637X/712/1/260 [arXiv:0907.1085 [astro-ph.GA]]
    
%\cite{Aprile:2018dbl}
\bibitem{Aprile:2018dbl} 
  E.~Aprile {\it et al.} [XENON Collaboration],
  %``Dark Matter Search Results from a One Ton-Year Exposure of XENON1T,''
  Phys.\ Rev.\ Lett.\  {\bf 121}, no. 11, 111302 (2018)
  doi:10.1103/PhysRevLett.121.111302
  [arXiv:1805.12562 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevLett.121.111302;%%
  %667 citations counted in INSPIRE as of 27 Mar 2020
  
%\cite{Freese:2012xd}
\bibitem{Freese:2012xd}
K.~Freese, M.~Lisanti and C.~Savage,
%``Colloquium: Annual modulation of dark matter,''
Rev.\ Mod.\ Phys.\  \textbf{85}, 1561-1581 (2013)
doi:10.1103/RevModPhys.85.1561
[arXiv:1209.3339 [astro-ph.CO]].
%244 citations counted in INSPIRE as of 07 Apr 2020

%\cite{Kelso:2013gda}
\bibitem{Kelso:2013gda}
C.~Kelso, P.~Sandick and C.~Savage,
%``Lowering the Threshold in the DAMA Dark Matter Search,''
JCAP \textbf{09}, 022 (2013)
doi:10.1088/1475-7516/2013/09/022
[arXiv:1306.1858 [astro-ph.CO]].
%14 citations counted in INSPIRE as of 07 Apr 2020

  %\cite{Bernabei:2008yh}
\bibitem{Bernabei:2008yh}
R.~Bernabei \textit{et al.} [DAMA],
%``The DAMA/LIBRA apparatus,''
Nucl. Instrum. Meth. A \textbf{592}, 297-315 (2008)
doi:10.1016/j.nima.2008.04.082
[arXiv:0804.2738 [astro-ph]].
%332 citations counted in INSPIRE as of 06 May 2020

%\cite{Bernabei:2008yi}
\bibitem{Bernabei:2008yi}
R.~Bernabei \textit{et al.} [DAMA],
%``First results from DAMA/LIBRA and the combined results with DAMA/NaI,''
Eur. Phys. J. C \textbf{56}, 333-355 (2008)
doi:10.1140/epjc/s10052-008-0662-y
[arXiv:0804.2741 [astro-ph]].
%1233 citations counted in INSPIRE as of 12 May 2020

%\cite{Bernabei:2010mq}
\bibitem{Bernabei:2010mq}
R.~Bernabei \textit{et al.} [DAMA and LIBRA],
%``New results from DAMA/LIBRA,''
Eur. Phys. J. C \textbf{67}, 39-49 (2010)
doi:10.1140/epjc/s10052-010-1303-9
[arXiv:1002.1028 [astro-ph.GA]].
%1035 citations counted in INSPIRE as of 12 May 2020
%\cite{Bernabei:2013xsa}
\bibitem{Bernabei:2013xsa} 
  R.~Bernabei {\it et al.},
  %``Final model independent result of DAMA/LIBRA-phase1,''
  Eur.\ Phys.\ J.\ C {\bf 73}, 2648 (2013)
  doi:10.1140/epjc/s10052-013-2648-7
  [arXiv:1308.5109 [astro-ph.GA]].
  %%CITATION = doi:10.1140/epjc/s10052-013-2648-7;%%
  %441 citations counted in INSPIRE as of 08 Apr 2020

%\cite{Bernabei:2018yyw}
\bibitem{Bernabei:2018yyw}
R.~Bernabei, P.~Belli, A.~Bussolotti, F.~Cappella, V.~Caracciolo, R.~Cerulli, C.~Dai, A.~d'Angelo, A.~Di Marco, H.~He, A.~Incicchitti, X.~Ma, A.~Mattei, V.~Merlo, F.~Montecchia, X.~Sheng and Z.~Ye,
%``First Model Independent Results from DAMA/LIBRA–Phase2,''
Universe \textbf{4}, no.11, 116 (2018)
doi:10.3390/universe4110116
[arXiv:1805.10486 [hep-ex]].
%107 citations counted in INSPIRE as of 07 Apr 2020


%\cite{Adhikari:2019off}
\bibitem{Adhikari:2019off}
G.~Adhikari \textit{et al.} [COSINE-100],
%``Search for a Dark Matter-Induced Annual Modulation Signal in NaI(Tl) with the COSINE-100 Experiment,''
Phys. Rev. Lett. \textbf{123}, no.3, 031302 (2019)
doi:10.1103/PhysRevLett.123.031302
[arXiv:1903.10098 [astro-ph.IM]].
%29 citations counted in INSPIRE as of 07 May 2020

%\cite{Abdelhameed:2019hmk}
\bibitem{Abdelhameed:2019hmk}
A.~Abdelhameed \textit{et al.} [CRESST],
%``First results from the CRESST-III low-mass dark matter program,''
Phys. Rev. D \textbf{100}, no.10, 102002 (2019)
doi:10.1103/PhysRevD.100.102002
[arXiv:1904.00498 [astro-ph.CO]].
%67 citations counted in INSPIRE as of 07 May 2020
\end{thebibliography}
\end{comment}
